New views of the distant stellar halo

Currently only a small number of Milky Way (MW) stars are known to exist beyond 100 kpc from the Galactic center. Though the distribution of these stars in the outer halo is believed to be sparse, they can provide evidence of more recent accretion events than in the inner halo and help map out the MW's dark matter halo to its virial radius. We have re-examined the outermost regions of 11 existing stellar halo models with two synthetic surveys: one mimicking present-day searches for distant M giants and another mimicking RR Lyrae (RRLe) projections for LSST. Our models suggest that color and proper motion cuts currently used to select M giant candidates for follow-up successfully remove nearly all halo dwarf self-contamination and are useful for focusing observations on distant M giants, of which there are thousands to tens of thousands beyond 100 kpc in our models. We likewise expect that LSST will identify comparable numbers of RRLe at these distances. We demonstrate that several observable properties of both tracers, such as proximity of neighboring stars, proper motions, and distances (for RRLe) could help us separate different accreted structures from one another. We also discuss prospects for using ratios of M giants to RRLe as a proxy for accretion time, which in the future could provide new constraints on the recent accretion history of our Galaxy.

==> JournalAbbrevs.tex <==
\newcommand\aj{{AJ}}% 
          % Astronomical Journal 
\newcommand\araa{{ARA\&A}}% 
          % Annual Review of Astron and Astrophys 
\newcommand\apj{{ApJ}}% 
          % Astrophysical Journal 
\newcommand\apjl{{ApJ}}% 
          % Astrophysical Journal, Letters 
\newcommand\apjs{{ApJS}}% 
          % Astrophysical Journal, Supplement 
\newcommand\ao{{Appl.~Opt.}}% 
          % Applied Optics 
\newcommand\apss{{Ap\&SS}}% 
          % Astrophysics and Space Science 
\newcommand\aap{{A\&A}}% 
          % Astronomy and Astrophysics 
\newcommand\aapr{{A\&A~Rev.}}% 
          % Astronomy and Astrophysics Reviews 
\newcommand\aaps{{A\&AS}}% 
          % Astronomy and Astrophysics, Supplement 
\newcommand\azh{{AZh}}% 
          % Astronomicheskii Zhurnal 
\newcommand\baas{{BAAS}}% 
          % Bulletin of the AAS 
\newcommand{\jcap}{J. Cosm. Astropart. Phys.}
	% Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{{JRASC}}% 
          % Journal of the RAS of Canada 
\newcommand\memras{{MmRAS}}% 
          % Memoirs of the RAS 
\newcommand\mnras{{MNRAS}}% 
          % Monthly Notices of the RAS 
\newcommand\pra{{Phys.~Rev.~A}}% 
          % Physical Review A: General Physics 
\newcommand\prb{{Phys.~Rev.~B}}% 
          % Physical Review B: Solid State 
\newcommand\prc{{Phys.~Rev.~C}}% 
          % Physical Review C 
\newcommand\prd{{Phys.~Rev.~D}}% 
          % Physical Review D 
\newcommand\pre{{Phys.~Rev.~E}}% 
          % Physical Review E 
\newcommand\prl{{Phys.~Rev.~Lett.}}% 
          % Physical Review Letters 
\newcommand\pasp{{PASP}}% 
          % Publications of the ASP 
\newcommand\pasj{{PASJ}}% 
          % Publications of the ASJ 
\newcommand\qjras{{QJRAS}}% 
          % Quarterly Journal of the RAS 
\newcommand\skytel{{S\&T}}% 
          % Sky and Telescope 
\newcommand\solphys{{Sol.~Phys.}}% 
          % Solar Physics 
\newcommand\sovast{{Soviet~Ast.}}% 
          % Soviet Astronomy 
\newcommand\ssr{{Space~Sci.~Rev.}}% 
          % Space Science Reviews 
\newcommand\zap{{ZAp}}% 
          % Zeitschrift fuer Astrophysik 
\newcommand\nat{{Nature}}% 
          % Nature 
\newcommand\iaucirc{{IAU~Circ.}}% 
          % IAU Cirulars 
\newcommand\aplett{{Astrophys.~Lett.}}% 
          % Astrophysics Letters 
\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}% 
          % Astrophysics Space Physics Research 
\newcommand\bain{{Bull.~Astron.~Inst.~Netherlands}}% 
          % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{{Fund.~Cosmic~Phys.}}% 
          % Fundamental Cosmic Physics 
\newcommand\gca{{Geochim.~Cosmochim.~Acta}}% 
          % Geochimica Cosmochimica Acta 
\newcommand\grl{{Geophys.~Res.~Lett.}}% 
          % Geophysics Research Letters 
\newcommand\jcp{{J.~Chem.~Phys.}}% 
          % Journal of Chemical Physics 
\newcommand\jgr{{J.~Geophys.~Res.}}% 
          % Journal of Geophysics Research 
\newcommand\jqsrt{{J.~Quant.~Spec.~Radiat.~Transf.}}% 
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand\memsai{{Mem.~Soc.~Astron.~Italiana}}% 
          % Mem. Societa Astronomica Italiana 
\newcommand\nphysa{{Nucl.~Phys.~A}}% 
          % Nuclear Physics A 
\newcommand\physrep{{Phys.~Rep.}}% 
          % Physics Reports 
\newcommand\physscr{{Phys.~Scr}}% 
          % Physica Scripta 
\newcommand\planss{{Planet.~Space~Sci.}}% 
          % Planetary Space Science 
\newcommand\procspie{{Proc.~SPIE}}% 
          % Proceedings of the SPIE 
\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 
